Scalable distributed service migration via Complex Networks Analysis

With social networking sites providing increasingly richer context, User-Centric Service (UCS) creation is expected to explode following a similar success path to User-Generated Content. One of the major challenges in this emerging highly user-centric networking paradigm is how to make these exploding in numbers yet, individually, of vanishing demand services available in a cost-effective manner. Of prime importance to the latter (and focus of this paper) is the determination of the optimal location for hosting a UCS. Taking into account the particular characteristics of UCS, we formulate the problem as a facility location problem and devise a distributed and highly scalable heuristic solution to it. Key to the proposed approach is the introduction of a novel metric drawing on Complex Network Analysis. Given a current location of UCS, this metric helps to a) identify a small subgraph of nodes with high capacity to act as service demand concentrators; b) project on them a reduced yet accurate view of the global demand distribution that preserves the key attraction forces on UCS; and, ultimately, c) pave the service migration path towards its optimal location in the network. The proposed iterative UCS migration algorithm, called cDSMA, is extensively evaluated over synthetic and real-world network topologies. Our results show that cDSMA achieves high accuracy, fast convergence, remarkable insensitivity to the size and diameter of the network and resilience to inaccurate estimates of demands for UCS across the network. It is also shown to clearly outperform local-search heuristics for service migration that constrain the subgraph to the immediate neighbourhood of the node currently hosting UCS.

==> conclusions.tex <==
\section{Conclusions and future work}
\label{Conclusions} In this paper we have developed a scalable and
effective approach in grappling with the complexity and
limitations of the distributed-fashion optimization of service
placement. The presented approach amounts to solving the
\textit{1-median} problem in a scalable manner by exploiting
information coming from the Complex Networks Analysis.

Regarding our work's next steps, we can identify the following two
-main- threads that seem worthwhile to investigate:
\begin{itemize}
 \item Relax the assumption that information-flow follows some certain kind of trajectories (i.e shortest path routes) to traverse the network. To this end, we need to devise new appropriate metrics to cope with the variation of information-flow characteristics (i.e. trails, walks)
 \item Take into account the practical cost of each migration hop and study -by forming a new optmization problem- its impact on the migration process; (\textit{namely, we aim to provide some guidelines on the number of the cost-effective migration hops given the constraint that the final provision cost plus the migration cost should not outgo the initial provision cost.})
\end{itemize}


==> mapping.tex <==
\section{Demand mapping}\label{sec:mapping}

The $wCBC(u,Host)$ metric lets us single out the subset of the ``most
appropriate'' nodes for solving the \textit{1-median} optimization problem.
Effectively, it assesses the ability of network nodes to act as
traffic demand concentrators. By selecting those few (preferably a
small percentage of the total number) with the top $wCBC(u,Host)$
values, no matter what their configuration around the current
$Host$ is, we solve our optimization on a subgraph (see Fig.~\ref{schematic}) formed
by those nodes that best reflect what ``amount"
of demand may come in -this subgraph- via different shortest paths
stemming from nodes, not included-in (the subgraph). As such, we end up with a
restricted in size optimization problem, taking into account both
\textit{precise} topology-demand information throughout the subgraph and
``outside coming-in'' demand, without actually knowing the
(exact value of) the latter. Note that a significant shift of the
demand load (for the available service) generated by some distant
node $y$, is captured \textit{implicitly} by the subgraph nodes $u$,
having some of them - that lie in between the node $y$ and the $Host$-
exhibit large $wCBC(u,Host)$ values;
$y$'s original (demand) value has been shaped by the
shortest paths ratio (as defined in eq.~\ref{eq3}).



%------------------------------ notes----------------------
%Consequently, the question of how sufficient is
%the information provided by the proposed CNA-based metric to help
%us clearly identify a cost-reducing path to move the service, is
%raised.

%The subgraph where small optimization takes place represented for the $i$-th iteration by
%$ G^{*(i)}$ where $ G \subseteq G^{*(i)} $
%Demand mapping: set a \textit{new }demand for the nodes taking part in the game that would reflect the demand coming from the rest of the nodes lying 'behind' them:

% By having exclusively the nodes $s\notin G^{*(i)}$ contribute to
% $selCBC(v;t)$ metric of each one $v$ to participate in the
% optimization, we are capable of catching the actual demand that
% would possibly pass-through without overestimating

